Planar Brownian Motion and Complex Analysis

A graduate level textbook on the interplay between complex analysis and Brownian motion.

==> chapter7.tex <==
\chapter{Evaluating contour integrals} \label{exittimes}

\section{Cauchy's integral formula and the residue theorem} \label{secexpectexit}

{\bf Proof:} As before, let $S_M = \inf\{t \geq 0:|B_t|=M\}$, and apply It\=o's Theorem to $-h$ to obtain

\begin{equation} \label{danp}
E_a[T_W \wedge S_M] = \frac{1}{2} \int_{0}^{T_W \wedge S_M} \Del (-h(B_s))ds = h(a) - E_a[h(B_{T_W \wedge S_M})] \leq h(a).
\end{equation}

Letting $M \nearrow \ff$, we obtain $E_a[T_W] \leq h(a) < \ff$. Once we know this, Burkholder's Theorem tells us that $E_a[|B_{T_W}^*|^2] < \ff$, which allows us to bound $h(B_{T_W \wedge S_M}) \leq C|B_{T_W \wedge S_M}|^2 + C \leq C|B^*_{T_W}|^2 + C$ and apply the Dominated Convergence Theorem in \rrr{danp} to obtain

\begin{equation} \label{}
E_a[T_W] = \lim_{M \nearrow \ff} E_a[T_W \wedge S_M] = h(a) - \lim_{M \nearrow \ff} E_a[h(B_{T_W \wedge S_M})] = h(a).
\end{equation}

\qed

We remark that the condition that $h$ be nonnegative is very important: in the example at the end of Section \ref{secexpectexit}, the function $h(a) = 1-|a|^2$ satisfies all of the other conditions in the theorem. The following theorem is a fairly general version of what is called the {\it Phragm\'en-Lindel\=of principle}. This principle is essentially a version of the maximum principle which is valid for functions which grow slowly on unbounded domains.

\begin{theorem} \label{phraglind1}
Let $W$ be a domain such that $E[T_W] < \ff$. Suppose that $f$ is an analytic function on $W$ such that $\limsup_{z \lar \dd W}|f(z)| \leq K < \ff$, and $|f(z)| \leq Ce^{C|z|^2} + C$. Then $|f(z)| \leq K$ for all $z \in W$.
\end{theorem}

We will need the following lemma. As usual, set $S_M = \inf\{t \geq 0:|B_t|=M\}$, and define

\begin{equation} \label{17dd}
\log^+ x = \begin{cases} \log x & x > 1,\\
0 & x  \leq 1.
\end{cases}
\end{equation}

\begin{lemma} \label{logpluslem}
If a function $f$ is analytic on a domain $W$ and continuous on $\CCC(W)$, then $\log^+ |f(a)| \leq E_a[\log^+|f(B_{T_W \wedge S_M})|]$.
\end{lemma}

{\bf Proof of Lemma \ref{logpluslem}:} We note first that, since $\log x$ and $g(x) = 0$ are both harmonic we have $\log |f(a)| = E_a[\log|f(B_{T_W \wedge S_M})|]$ and $g(|f(a)|) = E_a[g(|f(B_{T_W \wedge S_M})|)]$. Since $\log^+ = \max(\log, g)$, for any $a$ such that $\log^+ |f(a)| = \log |f(a)|$ we have $\log^+ |f(a)| = \log |f(a)| = E_a[\log|f(B_{T_W \wedge S_M})|] \leq E_a[\max(\log,g)(f(B_{T_W \wedge S_M}))] = E_a[\log^+(f(B_{T_W \wedge S_M}))]$. A similar calculation holds if $\log^+ |f(a)| = g(|f(a)|)$. \qed

{\bf Proof of Theorem \ref{phraglind1}:} By multiplying $f$ by a constant we may assume that $K=1$. The assumption on $f$ shows that $\log^+ |f(B_{T_W \wedge S_M})| \leq C|B_{T_W \wedge S_M}|^2 + C \leq C|B^*_{T_W \wedge S_M}|^2 + C$, and since $E[T_W] < \ff$ Burkholder's Theorem tells us that $E_a[C|B^*_{T_W \wedge S_M}|^2 + C] < \ff$. We may therefore apply the Dominated Convergence Theorem and Lemma \ref{17dd} to conclude

\begin{equation} \label{}
\log^+ |f(a)| \leq \lim_{M \nearrow \ff} E_a[\log^+|f(B_{T_W \wedge S_M})|] = E_a[\log^+|f(B_{T_W})|] = 1.
\end{equation}

Thus, $|f(a)| \leq 1$. \qed

{\bf Proof:} As before, let $S_M = \inf\{t \geq 0:|B_t|=M\}$, and apply It\=o's Theorem to $-h$ to obtain

\begin{equation} \label{danp}
E_a[T_W \wedge S_M] = \frac{1}{2} \int_{0}^{T_W \wedge S_M} \Del (-h(B_s))ds = h(a) - E_a[h(B_{T_W \wedge S_M})] \leq h(a).
\end{equation}

Letting $M \nearrow \ff$, we obtain $E_a[T_W] \leq h(a) < \ff$. Once we know this, Burkholder's Theorem tells us that $E_a[|B_{T_W}^*|^2] < \ff$, which allows us to bound $h(B_{T_W \wedge S_M}) \leq C|B_{T_W \wedge S_M}|^2 + C \leq C|B^*_{T_W}|^2 + C$ and apply the Dominated Convergence Theorem in \rrr{danp} to obtain

\begin{equation} \label{}
E_a[T_W] = \lim_{M \nearrow \ff} E_a[T_W \wedge S_M] = h(a) - \lim_{M \nearrow \ff} E_a[h(B_{T_W \wedge S_M})] = h(a).
\end{equation}

\qed

We remark that the condition that $h$ be nonnegative is very important: in the example at the end of Section \ref{secexpectexit}, the function $h(a) = 1-|a|^2$ satisfies all of the other conditions in the theorem. The following theorem is a fairly general version of what is called the {\it Phragm\'en-Lindel\=of principle}. This principle is essentially a version of the maximum principle which is valid for functions which grow slowly on unbounded domains.

\begin{theorem} \label{phraglind1}
Let $W$ be a domain such that $E[T_W] < \ff$. Suppose that $f$ is an analytic function on $W$ such that $\limsup_{z \lar \dd W}|f(z)| \leq K < \ff$, and $|f(z)| \leq Ce^{C|z|^2} + C$. Then $|f(z)| \leq K$ for all $z \in W$.
\end{theorem}

We will need the following lemma. As usual, set $S_M = \inf\{t \geq 0:|B_t|=M\}$, and define

\begin{equation} \label{17dd}
\log^+ x = \begin{cases} \log x & x > 1,\\
0 & x  \leq 1.
\end{cases}
\end{equation}

\begin{lemma} \label{logpluslem}
If a function $f$ is analytic on a domain $W$ and continuous on $\CCC(W)$, then $\log^+ |f(a)| \leq E_a[\log^+|f(B_{T_W \wedge S_M})|]$.
\end{lemma}

{\bf Proof of Lemma \ref{logpluslem}:} We note first that, since $\log x$ and $g(x) = 0$ are both harmonic we have $\log |f(a)| = E_a[\log|f(B_{T_W \wedge S_M})|]$ and $g(|f(a)|) = E_a[g(|f(B_{T_W \wedge S_M})|)]$. Since $\log^+ = \max(\log, g)$, for any $a$ such that $\log^+ |f(a)| = \log |f(a)|$ we have $\log^+ |f(a)| = \log |f(a)| = E_a[\log|f(B_{T_W \wedge S_M})|] \leq E_a[\max(\log,g)(f(B_{T_W \wedge S_M}))] = E_a[\log^+(f(B_{T_W \wedge S_M}))]$. A similar calculation holds if $\log^+ |f(a)| = g(|f(a)|)$. \qed

{\bf Proof of Theorem \ref{phraglind1}:} By multiplying $f$ by a constant we may assume that $K=1$. The assumption on $f$ shows that $\log^+ |f(B_{T_W \wedge S_M})| \leq C|B_{T_W \wedge S_M}|^2 + C \leq C|B^*_{T_W \wedge S_M}|^2 + C$, and since $E[T_W] < \ff$ Burkholder's Theorem tells us that $E_a[C|B^*_{T_W \wedge S_M}|^2 + C] < \ff$. We may therefore apply the Dominated Convergence Theorem and Lemma \ref{17dd} to conclude

\begin{equation} \label{}
\log^+ |f(a)| \leq \lim_{M \nearrow \ff} E_a[\log^+|f(B_{T_W \wedge S_M})|] = E_a[\log^+|f(B_{T_W})|] = 1.
\end{equation}

Thus, $|f(a)| \leq 1$. \qed

\section{Integrals on the real line}

The following lemma is basic but important for unbounded domains.

\begin{lemma} \label{}
\begin{itemize} \label{}

\item[(i)] Suppose $z \in W_1 \subseteq W_2$. Then $E_z[T_{W_1}] \leq E_z[T_{W_2}]$.

\item[(ii)] Suppose that $z \in W_1 \subseteq W_2 \subseteq \ldots$, and $W = \cup_{n=1}^\ff W_n$. Then $E_z[T_{W_n}] \nearrow E_z[T_{W}]$ as $n \lar \ff$.

\end{itemize}
\end{lemma}

{\bf Proof:} $(i)$ is obvious, and $(ii)$ is a simple consequence of the Monotone Convergence Theorem. \qed

The key to resolving the issues mentioned on unbounded domains is the following theorem, which is a special case of what we will refer to as {\it Burkholder's Theorem}, which can also be thought of as a planar form of the Davis Inequality. To state the theorem, we define the supremum process $|B^*_\tau| = \sup_{0 \leq t \leq \tau} |B_t|$ for any stopping time $\tau$. We then have

\begin{theorem} \label{burkthm}
For any stopping time $\tau$ we have

\begin{equation} \label{bteq}
2E_a[\tau] + |a|^2 \leq E_a[|B^*_\tau|^2] \leq 4(2E_a[\tau] + |a|^2).
\end{equation}
\end{theorem}

{\bf Proof:} First let us note that it is enough to prove the result in the case that $|B^*_\tau| \leq M$ a.s. This is because, if we do so, we can let $S_M = \inf\{t \geq 0:|B_t|=M\}$, apply the result to $\tau \wedge S_M$, and then let $M \nearrow \ff$, applying the Monotone Convergence Theorem to both $\tau \wedge S_M$ and $|B^*_{\tau \wedge S_M}|^2$ in order to obtain \rrr{bteq}. With this condition on $\tau$ we may apply It\=o's Theorem as in the proof of Proposition \ref{exitseries} to obtain $2E_a[\tau] + |a|^2 = E_a[|B_\tau|^2]$. It is clear that $E_a[|B_\tau|^2] \leq E_a[|B^*_\tau|^2]$, and we obtain the first inequality in \rrr{bteq}. The second follows similarly by utilizing the following important inequality.

\begin{proposition} \label{davisineq}
If $\tau$ is a stopping time with $E[\tau] < \ff$ then

\begin{equation} \label{}
E_a[|B^*_\tau|^2] \leq 4E_a[|B_\tau|^2].
\end{equation}
\end{proposition}

To prove this, we need several lemmas.

\begin{lemma} \label{}
\begin{equation} \label{}
E_a[|B_{S_M}|1_{S_M \leq \tau}] \leq E_a[|B_{\tau}|1_{S_M \leq \tau}]
\end{equation}
\end{lemma}

{\bf Proof:} Should follow from Dynkin's formula. \qed

\begin{lemma} \label{}
\begin{equation} \label{}
P_a(|B^*_\tau|\leq M) \leq \frac{1}{M} E_a[|B_\tau|1_{|B_\tau^*| \geq M}].
\end{equation}
\end{lemma}

{\bf Proof:}

\begin{equation} \label{}
P_a(|B^*_\tau|\leq M) = \frac{1}{M} E_a[|B_{S_M}|1_{S_M \leq \tau}] \leq \frac{1}{M} E_a[|B_{\tau}|1_{|B_\tau^*| \geq M}].
\end{equation}

\qed

\begin{lemma} \label{}
\begin{equation} \label{}
E[X^2] = \int_{0}^{\ff} 2M P(X > M) dM.
\end{equation}
\end{lemma}

{\bf Proof of Proposition \ref{davisineq}:}

\begin{equation} \label{}
\begin{split}
E_a[|B_\tau^*|^2 & = 2 \int_{0}^{\ff} M P(|B_\tau^*| > M) dM \\
& \leq 2 \int_{0}^{\ff} E_a[|B_\tau| 1_{|B_\tau^*| \geq M}]dM \\
& = 2 E_a[|B_\tau| \int_{0}^{|B_\tau^*|} dM] \\
& = 2 E_a[|B_\tau||B_\tau^*|] \\
& \leq E_a[|B_\tau|^2]^{1/2} E_a[|B_\tau^*|^2]^{1/2}.
\end{split}
\end{equation}

\qed

Armed with Burkholder's Theorem, we can impose a condition on harmonic functions on unbounded domains which will force them to be uniquely determined by their boundary values.

\begin{theorem} \label{phraglindharm}
Suppose $h$ is harmonic on a domain $W$ with $E[T_W] < \ff$ and continuous on $\CCC(W)$, with $h(z)= 0$ for $z \in \dd W$. If there is a constant $C>0$ such that $|h(z)| \leq C|z|^2 +C$, then $h(z) = 0$ for all $z \in W$.
\end{theorem}

{\bf Proof:} As in the proof of Theorem \ref{burkthm}, let $S_M = \inf\{t \geq 0:|B_t|=M\}$, and fix $a \in W$. By It\=o's Theorem, $h(a) = E_a[h(B_{T_W \wedge S_M})]$. We would like let $m \lar \ff$ to obtain $h(a) = E_a[h(B_{T_W})]=0$; note that the conditions on $h$ imply that $|h(B_{T_W \wedge S_M})| \leq C|B_{T_W \wedge S_M}|^2 + C \leq C|B^*_{T_W}|^2 + C$, and $E_a[C|B^*_{T_W}|^2 + C] \leq 4C (2E_a[T_W] + |a|^2) + C < \ff$ by Burkholder's Theorem. The Dominated Convergence Theorem therefore applies, and we get $h(a) = \lim_{M \nearrow \ff} E_a[h(B_{T_W \wedge S_M})] = E_a[h(B_{T_W})]=0$. \qed

This result suggests that our problem of determining the correct exit time function $h(a) = E_a[T_W]$ may be solved by imposing a growth condition on $h$, and this turns out to be correct.

\begin{theorem} \label{}
Suppose $W$ is a domain and $h$ is a nonnegative continuous function on $\CCC(W)$ such that $\Del h = -2$ on $W$ and $h = 0$ on $\dd W$. Suppose further that there is a constant $C>0$ such that $h(z) \leq C|z|^2 +C$. Then $E[T_W] < \ff$, and $h(a) = E_a[T_W]$ for all $a \in W$.
\end{theorem}

{\bf Proof:} As before, let $S_M = \inf\{t \geq 0:|B_t|=M\}$, and apply It\=o's Theorem to $-h$ to obtain

\begin{equation} \label{danp}
E_a[T_W \wedge S_M] = \frac{1}{2} \int_{0}^{T_W \wedge S_M} \Del (-h(B_s))ds = h(a) - E_a[h(B_{T_W \wedge S_M})] \leq h(a).
\end{equation}

Letting $M \nearrow \ff$, we obtain $E_a[T_W] \leq h(a) < \ff$. Once we know this, Burkholder's Theorem tells us that $E_a[|B_{T_W}^*|^2] < \ff$, which allows us to bound $h(B_{T_W \wedge S_M}) \leq C|B_{T_W \wedge S_M}|^2 + C \leq C|B^*_{T_W}|^2 + C$ and apply the Dominated Convergence Theorem in \rrr{danp} to obtain

\begin{equation} \label{}
E_a[T_W] = \lim_{M \nearrow \ff} E_a[T_W \wedge S_M] = h(a) - \lim_{M \nearrow \ff} E_a[h(B_{T_W \wedge S_M})] = h(a).
\end{equation}

\qed

We remark that the condition that $h$ be nonnegative is very important: in the example at the end of Section \ref{secexpectexit}, the function $h(a) = 1-|a|^2$ satisfies all of the other conditions in the theorem. The following theorem is a fairly general version of what is called the {\it Phragm\'en-Lindel\=of principle}. This principle is essentially a version of the maximum principle which is valid for functions which grow slowly on unbounded domains.

\begin{theorem} \label{phraglind1}
Let $W$ be a domain such that $E[T_W] < \ff$. Suppose that $f$ is an analytic function on $W$ such that $\limsup_{z \lar \dd W}|f(z)| \leq K < \ff$, and $|f(z)| \leq Ce^{C|z|^2} + C$. Then $|f(z)| \leq K$ for all $z \in W$.
\end{theorem}

We will need the following lemma. As usual, set $S_M = \inf\{t \geq 0:|B_t|=M\}$, and define

\begin{equation} \label{17dd}
\log^+ x = \begin{cases} \log x & x > 1,\\
0 & x  \leq 1.
\end{cases}
\end{equation}

\begin{lemma} \label{logpluslem}
If a function $f$ is analytic on a domain $W$ and continuous on $\CCC(W)$, then $\log^+ |f(a)| \leq E_a[\log^+|f(B_{T_W \wedge S_M})|]$.
\end{lemma}

{\bf Proof of Lemma \ref{logpluslem}:} We note first that, since $\log x$ and $g(x) = 0$ are both harmonic we have $\log |f(a)| = E_a[\log|f(B_{T_W \wedge S_M})|]$ and $g(|f(a)|) = E_a[g(|f(B_{T_W \wedge S_M})|)]$. Since $\log^+ = \max(\log, g)$, for any $a$ such that $\log^+ |f(a)| = \log |f(a)|$ we have $\log^+ |f(a)| = \log |f(a)| = E_a[\log|f(B_{T_W \wedge S_M})|] \leq E_a[\max(\log,g)(f(B_{T_W \wedge S_M}))] = E_a[\log^+(f(B_{T_W \wedge S_M}))]$. A similar calculation holds if $\log^+ |f(a)| = g(|f(a)|)$. \qed

{\bf Proof of Theorem \ref{phraglind1}:} By multiplying $f$ by a constant we may assume that $K=1$. The assumption on $f$ shows that $\log^+ |f(B_{T_W \wedge S_M})| \leq C|B_{T_W \wedge S_M}|^2 + C \leq C|B^*_{T_W \wedge S_M}|^2 + C$, and since $E[T_W] < \ff$ Burkholder's Theorem tells us that $E_a[C|B^*_{T_W \wedge S_M}|^2 + C] < \ff$. We may therefore apply the Dominated Convergence Theorem and Lemma \ref{17dd} to conclude

\begin{equation} \label{}
\log^+ |f(a)| \leq \lim_{M \nearrow \ff} E_a[\log^+|f(B_{T_W \wedge S_M})|] = E_a[\log^+|f(B_{T_W})|] = 1.
\end{equation}

Thus, $|f(a)| \leq 1$. \qed

\section{Advanced examples} \label{genmomsec}

Burkholder's Theorem admits a more general formulation.

\begin{theorem} \label{burkthm}
For any stopping time $\tau$ and $p \in (0,\ff)$ there are constants $c_p, C_p > 0$ such that

\begin{equation} \label{bteq}
c_pE_a[(\tau + |a|^2)^p] \leq E_a[|B^*_\tau|^{2p}] \leq C_p E_a[(\tau + |a|^2)^p].
\end{equation}

In particular, $E_a[\tau^p] < \ff$ if, and only if, $E_a[|B^*_\tau|^{2p}]< \ff$.
\end{theorem}

The proofs of Theorems \ref{phraglindharm} and \ref{phraglind1} are easily adapted, using this more general result, and yield the following results.

\begin{theorem} \label{phraglindharm2}
Suppose $h$ is harmonic on a domain $W$ with $E[T^p_W] < \ff$ and continuous on $\CCC(W)$, with $h(z)= 0$ for $z \in \dd W$. If there is a constant $C>0$ such that $|h(z)| \leq C|z|^{2p} +C$, then $h(z) = 0$ for all $z \in W$.
\end{theorem}

\begin{theorem} \label{phraglind2}
Let $W$ be a domain such that $E[T^p_W] < \ff$. Suppose that $f$ is an analytic function on $W$ such that $\limsup_{z \lar \dd W}|f(z)| \leq K < \ff$, and $|f(z)| \leq Ce^{C|z|^{2p}} + C$. Then $|f(z)| \leq K$ for all $z \in W$.
\end{theorem}

\section{Exercises}

\ccases{idententire} a) Find all entire functions $f(z)$ such that $f(1/n) = 1/n^2$ for all $n \in \NN$.

b) Find all entire functions $f(z)$ such that $f(1/n) = 1/\sqrt{n}$ for all $n \in \NN$.

\vski

\ccases{openaxes} Suppose $f(z)$ is an analytic function on a domain $W$ with the property that $f(z)^n \in \RR$ for all $z \in W$. Show that $f$ is a constant function.

\vski

\ccases{lindprep} Suppose that $\ga$ is a {\it Jordan curve}: that is, $\ga$ can be realized as the image of a continuous and one-to-one function $\ga(t)$ from $[0,1]$ into $\CC$. $\ga$ then determines a bounded domain $W$ in its interior. Suppose that $f(z)$ is an analytic function on $W$, and suppose that there are points $w_1, \ldots , w_n \in \ga$ such that $\limsup_{\{z \lar \dd W \backslash \{w_1, \ldots ,w_n\}\}} |f(z)| \leq m < \ff$. Suppose further that there is some finite $M > m$ such that $|f(z)| \leq M$ for all $z \in W$. Show that in fact $|f(z)| \leq m$ for all $z \in W$.

\hspace{1.2in} \includegraphics[width=90mm,height=70mm]{Lindelof.pdf}

\vski

\ccases{rotatethis} Let $W$ be the square domain $\{-1<x<1,-1<y<1\}$. Suppose $f(z)$ is a bounded analytic function on $W$ such that $f(z) \lar 0$ as $z$ approaches the bottom edge of the square; that is, $\lim_{\{z \lar \{y=-1\}\}} |f(z)| = 0$. Prove that $f(z) = 0$ for all $z \in W$.

\vski


\ccases{k-roots} Suppose $p(z) = \bb_k z^k + \ldots + \bb_0$ is a degree $k$ polynomial, with $\bb_0, \ldots, \bb_k \in \CC$ and $\bb_k \neq 0$. Show that $p$ has $k$ roots, counting multiplicities. That is, show that there are values $a_1, \ldots, a_k, c \in \CC$ such that $p(z) = c(z-a_1)(z-a_2)\ldots (z-a_k)$. (Hint: If $p(a) = 0$, consider $p(z)-p(a)$).

\vski

\ccases{intprop} i) (Independence of parameterizations) Suppose $\ga_1: [a_1,b_1] \lar \CC$ and $\ga_2: [a_2,b_2] \lar \CC$ are rectifiable curves, and suppose that there is a smooth increasing function $\phi : [a_1,b_1] \lar [a_2,b_2]$ with $\phi(a_1) = a_2, \phi(b_1) = b_2$ such that $\ga_1(t) = \ga_2(\phi(t))$ for all $t \in [a_1,b_1]$. Show that

\begin{equation} \label{}
\int_{\ga_1} f(z)dz = \int_{\ga_2} f(z)dz
\end{equation}
%
for any analytic function $f$ defined in a neighborhood of $\ga_1=\ga_2$.

\vski

ii) (Path reversal) Let $\ga: [a_1,b_1] \lar \CC$ be a rectifiable curve. Define $\tilde \ga : [-b_1,-a_1] \lar \CC$ by $\tilde \ga (t) = \ga (-t)$. Then $\tilde \ga$ is simply the curve $\ga$ traversed in the opposite direction. Show that

\begin{equation} \label{}
\int_{\tilde \ga} f(z)dz = - \int_{\ga} f(z)dz
\end{equation}
%
for any analytic function $f$ defined in a neighborhood of $\ga$.

\vski

iii) (Concatenating paths) Suppose $\ga_1: [a,b] \lar \CC$ and $\ga_2: [c,d] \lar \CC$ are rectifiable curves such that $\ga_1(b) = \ga_2(c)$. Define a new curve $\tilde \ga: [a, b+d-c] \lar \CC$ by

\begin{equation} \label{17}
\tilde \ga(t) := \begin{cases} \ga_t(t) & t \in [a,b],\\
\ga_2(t-b+c) & t \in [b,b+d-c].
\end{cases}
\end{equation}
%
$\tilde \ga$ is the concatenation of $\ga_1$ and $\ga_2$. Show that

\begin{equation} \label{}
\int_{\tilde \ga} f(z)dz = \int_{\ga_1} f(z)dz + \int_{\ga_2} f(z)dz
\end{equation}
%
for any analytic function $f$ defined in a neighborhood of $\tilde \ga$.

\vski

\ccases{compdist} Let $d(z,\dd W)$ be as in Section \ref{CTsec}. Show that the function $z \lar d(z,\dd W)$ is continuous and positive on $W$. Conclude that if $K$ is a compact set in $W$ then there is some $\eps > 0$ such that $d(z,\dd W) > 0$ for all $z \in K$.

\vski

\ccases{radconvsame} Show that the radius of convergence is the same for the three series $\sum_{n=0}^{\ff} \bb_n (z-z_0)^n, \sum_{n=0}^{\ff} \frac{\bb_n}{n+1} (z-z_0)^{n+1},$ and $\sum_{n=1}^{\ff} n \bb_n (z-z_0)^{n-1}$.

\vski

\ccases{polytriang} Polygon admits triangulation.

{\bf \Large 1.} Let $\ga = \{e^{it}: 0 \leq t \leq 2\pi\}$. Evaluate the following two integrals.

\begin{equation} \label{}
\int_{\ga} \frac{1}{z}dz, \qquad \int_{\ga} \frac{1}{z^2}dz.
\end{equation}

{\bf \Large 2.} Let $\ga(t): [0, 5\pi]$ be defined as follows.

\begin{equation} \label{17}
\ga(t) = \begin{cases} (t+\frac{3\pi}{2})e^{it} & 0 \leq t \leq 2 \pi,\\
\frac{3\pi}{2} + 2\pi e^{-it} & 2\pi \leq t \leq 3 \pi,\\
(t-\frac{7 \pi}{2}) + i \cos (t-\frac{7 \pi}{2}) & 3 \pi \leq t \leq 5\pi.
\end{cases}
\end{equation}

Sketch $\ga$, and evaluate

\begin{equation} \label{}
\int_{\ga} e^{1/z} dz .
\end{equation}

{\bf \Large 3.}  Suppose $p(z) = \bb_k z^k + \ldots + \bb_0$ is a degree $k$ polynomial, with $\bb_0, \ldots, \bb_k \in \CC$ and $\bb_k \neq 0$. Show that $p$ has $k$ roots, counting multiplicities. That is, show that there are values $a_1, \ldots, a_k, c \in \CC$ such that $p(z) = c(z-a_1)(z-a_2)\ldots (z-a_k)$. (Hint: If $p(a) = 0$, consider $p(z)-p(a)$).

\ccases{exlineremove} Suppose $W$ is a domain and $C$ is a line intersecting $W$. Suppose further that $f$ is a continuous function on $W$ which is analytic on $W \bsh C$. Show that in fact $f$ is analytic on all of $W$. (Hint: Morera's Theorem)

